Bound states in the B-matrix formalism for the three-body scattering

We consider a model of relativistic three-body scattering with a bound state in the two-body sub-channel. We show that the na\"ive K-matrix type parametrization, here referred to as the B-matrix, has nonphysical singularities near the physical region. We show how to eliminate such singularities by using dispersion relations and also show how to reproduce unitarity relations by taking into account all relevant open channels.

==> diagram.tex <==
% one vertex diagrams 20mm and (55,40)
% two vertices diagrams 38mm and (110,40)
% vertex size 20pt
% two-body circle size 0.14w and 0.07w

\begin{fmffile}{vertices}
    \beq
    \nonumber
    \parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v1}
	%Propagators
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*} }
	%%%
	&=&
	%%%
	\parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{22}$, label.dist=0pt,decor.size=20pt}{v1}
	%Propagators
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*}}
	%%%
	+
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{22}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	%Propagator
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes, left=0.8, tension=0.5}{v1,v2}
	\fmf{plain, right=-0.8, tension=0.5}{v2,v1}
	\fmf{dashes}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	+
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{23}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	%Propagator
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain,left=0.8, tension=0.5}{v1,v2}
	\fmf{plain, right=-0.8, tension=0.5}{v2,v1}
	\fmf{dashes}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	\\[10pt]
	%%%%%%%%%%%%%%%%%%%%
	%NEW LINE %A23
	%%%%%%%%%%%%%%%%%%%%
	\nonumber
    \parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v1}
	%Propagators
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*} }
	%%%
	&=&
	%%%
	\parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{23}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=0.15w}{f}
	\fmfforce{(0.5w,0.5h)}{v1}
	\fmfforce{(0.76w,0.82h)}{f}
	%Propagators
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain}{v1,f,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*}}
	%%%
	+
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{22}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	%Propagator
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes, left=0.8, tension=0.5}{v1,v2}
	\fmf{plain, right=-0.8, tension=0.5}{v2,v1}
	\fmf{dbl_plain}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	+
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{23}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	%Propagator
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain,left=0.8, tension=0.5}{v1,v2}
	\fmf{plain, right=-0.8, tension=0.5}{v2,v1}
	\fmf{dbl_plain}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	\\[10pt]
	%%%%%%%%%%%%%%%%%%%%
	%NEW LINE A32
	%%%%%%%%%%%%%%%%%%%%
	\nonumber
    \parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v1}
	%Propagators
	\fmf{dbl_plain}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*} }
	%%%
	&=&
	%%%
	\parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{32}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=0.14w}{f}
	\fmfforce{(0.5w,0.5h)}{v1}
	\fmfforce{(0.24w,0.82h)}{f}
	%Propagators
	\fmf{dbl_plain}{i2,f,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*}}
	%%%
	+
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{32}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=0.07w}{f}
	\fmfforce{(0.3w,0.5h)}{v1}
	\fmfforce{(0.17w,0.82h)}{f}
	%Propagator
	\fmf{dbl_plain}{i2,f,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes, left=0.8, tension=0.5}{v1,v2}
	\fmf{plain, right=-0.8, tension=0.5}{v2,v1}
	\fmf{dashes}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	+
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{33}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=0.07w}{f}
	\fmfforce{(0.3w,0.5h)}{v1}
	\fmfforce{(0.17w,0.82h)}{f}
	%Propagator
	\fmf{dbl_plain}{i2,f,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain,left=0.8, tension=0.5}{v1,v2}
	\fmf{plain, right=-0.8, tension=0.5}{v2,v1}
	\fmf{dashes}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	\\[10pt]
	%%%%%%%%%%%%%%%%%%%%
	%NEW LINE
	%%%%%%%%%%%%%%%%%%%%
	\nonumber
    \parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v1}
	%Propagators
	\fmf{dbl_plain}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*} }
	%%%
	&=&
	%%%
	\parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{33}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=0.14w}{f1,f2}
	\fmfforce{(0.5w,0.5h)}{v1}
	\fmfforce{(0.24w,0.82h)}{f1}
	\fmfforce{(0.76w,0.82h)}{f2}
	%Propagators
	\fmf{dbl_plain}{i2,f1,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain}{v1,f2,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*}}
	%%%
	+
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{32}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=0.07w}{f1}
	\fmfforce{(0.3w,0.5h)}{v1}
	\fmfforce{(0.17w,0.82h)}{f1}
	\fmfforce{(0.7w,0.5h)}{v2}
	%Propagator
	\fmf{dbl_plain}{i2,f1,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes, left=0.8, tension=0.5}{v1,v2}
	\fmf{plain, right=-0.8, tension=0.5}{v2,v1}
	\fmf{dbl_plain}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	+
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=empty, label=$\mathcal{B}_{33}$, label.dist=0pt,decor.size=20pt}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=20pt}{v2}
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=0.07w}{f1}
	\fmfforce{(0.3w,0.5h)}{v1}
	\fmfforce{(0.17w,0.82h)}{f1}
	\fmfforce{(0.7w,0.5h)}{v2}
	%Propagator
	\fmf{dbl_plain}{i2,f1,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain, left=0.8, tension=0.5}{v1,v2}
	\fmf{plain, right=-0.8, tension=0.5}{v2,v1}
	\fmf{dbl_plain}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
\eeq
\end{fmffile}

==> diagram_2.tex <==

\begin{fmffile}{vertices}
    \beq
    \nonumber
    \parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=6pt,label=$~g_{22}$}{v1}
	%Propagators
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dashes}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*} }
	%%%
	&=&
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=6pt,label=$\hspace{-25pt} \eta$}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=6pt,label=$~\eta$}{v2}
	%Propagator
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{zigzag}{v1,v2}
	\fmf{dashes}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	\\[10pt]
	%%%%%%%%%%%%%%%%%%%%
	%NEW LINE %A23
	%%%%%%%%%%%%%%%%%%%%
	\nonumber
    \parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=6pt,label=$~g_{32}$}{v1}
	%Propagators
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*} }
	%%%
	&=&
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=6pt,label=$\hspace{-25pt} \lambda$}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=6pt,label=$~\eta$}{v2}
	%Propagator
	\fmf{dashes}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{zigzag}{v1,v2}
	\fmf{dbl_plain}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
	\\[10pt]
	%%%%%%%%%%%%%%%%%%%%
	%NEW LINE A32
	%%%%%%%%%%%%%%%%%%%%
	\nonumber
    \parbox{20mm}{
	\begin{fmfgraph*}(55,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=6pt,label=$~g_{33}$}{v1}
	%Propagators
	\fmf{dbl_plain}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{dbl_plain}{v1,o2}
	\fmf{plain}{v1,o1}
	\end{fmfgraph*} }
	%%%
	&=&
	%%%
	\parbox{38mm}{
	\begin{fmfgraph*}(110,40)
	%Vertices left
	\fmfleft{i1,i2} 
	%Vertices right
	\fmfright{o1,o2}
	%Internal vertices
	\fmfv{decor.shape=circle,decor.filled=full, label.dist=0pt,decor.size=6pt,label=$\hspace{-25pt} \lambda$}{v1}
	\fmfv{decor.shape=circle,decor.filled=full, decor.size=6pt,label=$~\lambda$}{v2}
	%Propagator
	\fmf{dbl_plain}{i2,v1}
	\fmf{plain}{i1,v1}
	\fmf{zigzag,zigzag_width=0.02}{v1,v2}
	\fmf{dbl_plain}{v2,o2}
	\fmf{plain}{v2,o1}
	\end{fmfgraph*}}
	%%%
\eeq
\end{fmffile}

